SHIELD: An Adaptive and Lightweight Defense against the Remote Power Side-Channel Attacks on Multi-tenant FPGAs

Dynamic partial reconfiguration enables multi-tenancy in cloud-based FPGAs, which presents security challenges for tenants, IPs, and data. Malicious users can exploit FPGAs for remote side-channel attacks (SCAs), and shared on-chip resources can be used for attacks. Logical separation can ensure design integrity, but on-chip resources can still be exploited. Conventional SCA mitigation can help, but it requires significant effort, and bitstream checking techniques are not highly accurate. An active on-chip defense mechanism is needed for tenant confidentiality. Toward this, we propose a lightweight shielding technique utilizing ring oscillators (ROs) to protect applications against remote power SCA. Unlike existing RO-based approaches, in our methodology, an offline pre-processing stage is proposed to carefully configure power monitors and an obfuscating circuit concerning the resource constraints of the board. Detection of power fluctuations due to application execution enables the obfuscating circuit to flatten the power consumption trace. To evaluate the effectiveness of the proposed SHIELD, we implemented it on a Xilinx Zynq-7000 FPGA board executing an RSA encryption algorithm. Due to the SHIELD, the number of traces required to extract the encryption key is increased by 166x, making an attack extremely hard at run-time. Note that the proposed SHIELD does not require any modification in the target application. Our methodology also shows up to 54% less power consumption and up to 26% less area overhead than the state-of-the-art random noise-addition-based defense.

==> Sections/Table.tex <==

\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}

==> settings.tex <==
\IEEEoverridecommandlockouts
% The preceding line is only needed to identify funding in the first footnote. If that is unneeded, please comment it out.
%=================================================================================
\ifCLASSINFOpdf
%
\else
%  
\fi
% 
% ----------------------------- FORMATTING START ---------------------------------
\usepackage[letterpaper]{geometry}
%\newgeometry{left=1.57cm,right=1.57cm,bottom=2.54cm,top=2.0cm} %ORIGINAL
% %\newgeometry{left=1.57cm,right=1.57cm,bottom=2.0cm,top=1.6cm}
\newgeometry{left=1.5cm,right=1.5cm,bottom=2.0cm,top=1.5cm}
%\newgeometry{left=1.35cm,right=1.35cm,bottom=1.35cm,top=1.35cm}

% % change linespacing:
\usepackage{setspace}
\setstretch{0.91} % smaller
% % ----------------------------- FORMATTING END ---------------------------------

\usepackage{cite}
\usepackage[font=footnotesize]{caption}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage{algpseudocode}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{float}
%\usepackage[a4paper, total={184mm,239mm}]{geometry}
\usepackage{enumitem}
\usepackage[implicit=false,hidelinks]{hyperref}
%% ----------------------------- PACKAGES END ---------------------------------

\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
%% ----------------------------- Footnote line ---------------------------------    
\makeatletter
\renewcommand\footnoterule{%
  \kern-3\p@
  \hrule\@width 0.5\columnwidth
  \kern2.6\p@}
  \makeatother
  
\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}

\algnewcommand\algorithmicoutput{\textbf{Output:}}
\algnewcommand\Output{\item[\algorithmicoutput]}

\algnewcommand\algorithmicinitialize{\textbf{Initialize:}}
\algnewcommand\Initialize{\item[\algorithmicinitialize]}

\let\oldReturn\Return
\renewcommand{\Return}{\State\oldReturn}

  
\setlength{\textfloatsep}{3pt}
\setlength{\floatsep}{3pt}


\renewcommand{\IEEEbibitemsep}{0.5pt}
\makeatletter
\IEEEtriggercmd{\reset@font\normalfont\fontsize{8pt}{10pt}\selectfont}
%\IEEEtriggercmd{\reset@font\normalfont\fontsize{6.8pt}{7.11pt}\selectfont}
\makeatother
\IEEEtriggeratref{1}


